SpectroMotion: Dynamic 3D Reconstruction of Specular Scenes

We present SpectroMotion, a novel approach that combines 3D Gaussian Splatting (3DGS) with physically-based rendering (PBR) and deformation fields to reconstruct dynamic specular scenes. Previous methods extending 3DGS to model dynamic scenes have struggled to represent specular surfaces accurately. Our method addresses this limitation by introducing a residual correction technique for accurate surface normal computation during deformation, complemented by a deformable environment map that adapts to time-varying lighting conditions. We implement a coarse-to-fine training strategy significantly enhancing scene geometry and specular color prediction. It is the only existing 3DGS method capable of synthesizing photorealistic real-world dynamic specular scenes, outperforming state-of-the-art methods in rendering complex, dynamic, and specular scenes.

==> figs/gamma.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/gamma.pdf}
    \caption{\textbf{Qualitative comparison on different $\gamma^k$.}}
    \label{fig:gamma}
\end{figure*} 

==> figs/normal_weight.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/normal_weight.pdf}
    \caption{\textbf{Qualitative comparison on different $\lambda_{\text{normal}}$.}}
    \label{fig:lambda_normal}
\end{figure*} 

==> figs/select_checkpoint.tex <==
\begin{figure}[ht]
    \vspace{-2mm}
    \centering
    \includegraphics[width=1\linewidth]
    {figures/select_checkpoint_result.pdf}
    % \caption{Qualitative comparison between our method and Deformable 3DGS using the best checkpoint selection criterion.} 
    % \label{fig:select_checkpoint_result}
    \vspace{-10mm}
\end{figure}

==> figs/waymo_compare.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]
    {figures/waymo_compare.pdf}
    \caption{\textbf{Comparison of our method and Deformable 3DGS on reflective cars.}} 
    \label{fig:waymo_compare}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/gamma.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Ablation study on different $\gamma^k$}}
\label{tab:gamma}
\begin{tabular}{lccc}
    \toprule
      & PSNR ↑ & SSIM ↑ & LPIPS ↓ \\
    \midrule
    $\gamma^k, \quad k = 0$ &24.09  &0.8515  &0.1818  \\
    $\gamma^k, \quad k = 1$ &24.14  &\textbf{0.8523}  &0.1786  \\
    $\gamma^k, \quad k = 5$ &\textbf{24.17}  &0.8522  &\textbf{0.1778}  \\
    $\gamma^k, \quad k = 50$ & 24.11  & 0.8521  &0.1793  \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/hypernerf.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{3pt}
    \centering
    % \tiny
    \caption{\textbf{Quantitative comparison on the HyperNeRF~\citep{park2021hypernerf} dataset.} We report the average PSNR, SSIM, and LPIPS (VGG) of several previous models. The \colorbox{red!25}{best}, the \colorbox{orange!25}{second best}, and \colorbox{yellow!25}{third best} results are denoted by red, orange, yellow. }
    \label{tab:hypernerf}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccccccccccccccccccc}
    \toprule
     & \multicolumn{3}{c}{Broom} & &\multicolumn{3}{c}{3D printer}& &\multicolumn{3}{c}{Chicken}& &\multicolumn{3}{c}{Peel Banana}& &\multicolumn{3}{c}{\textbf{Mean}} \\ \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}\cmidrule{18-20}
    Method & PSNR↑ & SSIM↑& LPIPS↓& &PSNR↑ & SSIM↑& LPIPS↓& &PSNR↑ & SSIM↑& LPIPS↓& &PSNR↑ & SSIM↑& LPIPS↓& &PSNR↑ & SSIM↑& LPIPS↓  \\ 
    \midrule
    Deformable 3DGS~\citep{yang2023deformable} &\colorbox{yellow!25}{20.87} &{0.3202} &{0.5985} & &20.35&{0.6673}&\colorbox{orange!25}{0.3091} & &{22.63}&{0.6346} &\colorbox{red!25}{0.2616} & &\colorbox{orange!25}{27.27} &\colorbox{red!25}{0.8584} &\colorbox{red!25}{0.1828}& &{22.78} &{0.6201} &\colorbox{orange!25}{0.3380} \\ 
    4DGS~\citep{wu20234d} &\colorbox{orange!25}{21.21} &\colorbox{yellow!25}{0.3555} &\colorbox{yellow!25}{0.5669} & &\colorbox{yellow!25}{21.90} &\colorbox{orange!25}{0.6993} &0.3198& &\colorbox{red!25}{28.69} &\colorbox{red!25}{0.8143} &\colorbox{orange!25}{0.2772} & &\colorbox{red!25}{27.77} &\colorbox{yellow!25}{0.8431} &\colorbox{yellow!25}{0.2049}& &\colorbox{red!25}{24.89} &\colorbox{red!25}{0.6781} &\colorbox{yellow!25}{0.3422} \\
    GaussianShader~\citep{jiang2023gaussianshader} &17.21 &0.2263 &0.5812 & &17.31 &0.5926 &0.5054 & &19.70 &0.6520 &0.5004 & &19.99 &0.7097 &0.3308& &18.55 &0.5452 &0.4795 \\
    GS-IR~\citep{liang2023gs} &20.46 &0.3420 &\colorbox{red!25}{0.5229} & &18.24 &0.5745 &0.5204 & &20.64 &0.6592 &0.4536 & &20.15 &{0.7159} &{0.3021}& &19.87 &0.5729 &0.4498 \\
    NeRF-DS~\citep{yan2023nerf} &\colorbox{red!25}{22.37} &\colorbox{red!25}{0.4371} &0.5694 & &\colorbox{red!25}{22.16} &\colorbox{yellow!25}{0.6973} &\colorbox{yellow!25}{0.3134} & &\colorbox{yellow!25}{27.32} &\colorbox{yellow!25}{0.7949} &0.3139 & &{22.75} &0.6328 &0.3919& &\colorbox{orange!25}{23.65} &\colorbox{orange!25}{0.6405} &0.3972 \\
    HyperNeRF~\citep{park2021hypernerf} &20.72 &\colorbox{orange!25}{0.4276} &0.5773 & &\colorbox{orange!25}{21.94} &\colorbox{red!25}{0.7003} &\colorbox{red!25}{0.3090} & &\colorbox{orange!25}{27.40} &\colorbox{orange!25}{0.8013} &{0.3052} & &22.36 &0.6257 &0.3956& &\colorbox{yellow!25}{23.11} &\colorbox{yellow!25}{0.6387} &{0.3968} \\
    Ours &{20.24} &{0.3019} &\colorbox{orange!25}{0.5253} & &20.03 &0.6596 &{0.3206} & &21.70 &0.6225 &\colorbox{yellow!25}{0.2807} & &\colorbox{yellow!25}{26.91} &\colorbox{orange!25}{0.8510} &\colorbox{orange!25}{0.1914}& &22.22 &{0.6088} &\colorbox{red!25}{0.3295} \\ 
    \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/improve.tex <==
\newcommand{\best}[1]{{\textbf{\textcolor{red}{#1}}}}
\newcommand{\second}[1]{{\underline{\textcolor{blue}{#1}}}}

\begin{table}[ht]
\vspace{-1.5mm}
\centering
\footnotesize
% \caption{Comparison of improvements among our method, Deformable 3DGS, and GaussianShader.}
\label{tab:improve}
\vspace{-2mm}
\begin{tabular}{lccc}
\toprule
Method & $\Delta$PSNR  & $\Delta$SSIM  & $\Delta$LPIPS  \\
\midrule
GaussianShader (CVPR'24)&-0.94 &-0.0120 &+0.0040 \\
Deformable 3DGS (CVPR'24)&+0.51 &+0.0031 &+0.0047 \\
Ours (best checkpoint)&\best{+1.19} &\best{+0.0159} &\second{+0.0080}\\
Ours (40k iterations)&\second{+0.74} &\second{+0.0145} &\best{+0.0337}\\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

==> tables/lambda_normal.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Ablation study on different $\lambda_{\text{normal}}$}}
\label{tab:lambda_normal}
\begin{tabular}{lccc}
    \toprule
      & PSNR ↑ & SSIM ↑ & LPIPS ↓ \\
    \midrule
    $\lambda_{\text{normal}} = 1$ &8.35  &0.1031  &0.5954  \\
    $\lambda_{\text{normal}} = 0.1$ &15.14  &0.4379  &0.4529  \\
    $\lambda_{\text{normal}} = 0.01$ &\textbf{24.17}  &\textbf{0.8522}  &\textbf{0.1778}  \\
    $\lambda_{\text{normal}} = 0.001$ & 24.13  & 0.8522  &0.1796  \\
    $\lambda_{\text{normal}} = 0.0001$ & 24.10  & 0.8520  &0.1803  \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/select_checkpoint.tex <==
\begin{table}[ht]
\vspace{-1.5mm}
\centering
\scriptsize
% \caption{Quantitative comparison between our method and Deformable 3DGS using the best checkpoint selection criterion.}
% \label{tab:select_checkpoint}
\vspace{-2mm}
\begin{tabular}{lccc}
\toprule
Method & PSNR ↑ & SSIM ↑ & LPIPS ↓ \\
\midrule
Deformable 3DGS (original paper) &24.11 &0.8525 &0.1769 \\
Ours (best checkpoint) &\textbf{25.30} &\textbf{0.8684} &\textbf{0.1689}\\
% Deformable 3DGS (background) &25.10 &0.8834 &0.1618 \\
% Ours (background) &25.33 &0.8849 &0.1613 \\
% Deformable 3DGS (foreground) & & & \\
% Ours (foreground) & & & \\
\bottomrule
\end{tabular}
\vspace{-6mm}
\end{table}
